3D-R2N2: A Unified Approach for Single and Multi-view 3D Object Reconstruction

Inspired by the recent success of methods that employ shape priors to achieve robust 3D reconstructions, we propose a novel recurrent neural network architecture that we call the 3D Recurrent Reconstruction Neural Network (3D-R2N2). The network learns a mapping from images of objects to their underlying 3D shapes from a large collection of synthetic data. Our network takes in one or more images of an object instance from arbitrary viewpoints and outputs a reconstruction of the object in the form of a 3D occupancy grid. Unlike most of the previous works, our network does not require any image annotations or object class labels for training or testing. Our extensive experimental analysis shows that our reconstruction framework i) outperforms the state-of-the-art methods for single view reconstruction, and ii) enables the 3D reconstruction of objects in situations when traditional SFM/SLAM methods fail (because of lack of texture and/or wide baseline).

==> figures/mv_lstm_multiview.tex <==
\newcommand\wxk{0.092}
\begin{figure}
\begin{tabular}{cccccccccc}
  %row 1, images
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/4} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/4} \\
  %row 1, reconstructions
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane1_5/5_pred} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/plane4_5/5_pred} \\    

  %row 2, images

  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/4} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/4} \\
  %row 2, reconstructions


  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car1_5/5_pred} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/car5_5/5_pred} \\    

  
  
  %row 3, images
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/4} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/4} \\
  %row 3, reconstructions
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/bench1_5/5_pred} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/chair1_5/5_pred} \\    
 
   %row 4, images
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/4} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/0} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/1} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/2} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/3} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/4} \\
  %row 4, reconstructions
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/firearm1_5/5_pred} &
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/1_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/2_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/3_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/4_pred} &  
  \includegraphics[width=\wxk\linewidth]{figures/mv_lstm_multiview/lamp1_5/5_pred} \\    

 
\end{tabular}
\label{fig:multiview_qualitative}
\caption{Sample reconstruction on the ShapeNet dataset}
\end{figure}


==> figures/res_net_ebay/figure.tex <==
\newcommand\wxebay{0.085}
\newcommand\wxebayfail{0.078}

\begin{figure}
\vspace{\figurevspace}
\begin{center}
\begin{tabular}{cccccccccc}
  %row 1, images
  &\includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/121704583154/0} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/121704583154/1} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/121704583154/2} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/141395654974/0} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/141395654974/1} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/141395654974/2} &
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/381068411290/0} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/381068411290/1} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/381068411290/2} \\
  %row 1, reconstructions
  (a) &\includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/121704583154/0_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/121704583154/1_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/121704583154/2_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/141395654974/0_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/141395654974/1_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/141395654974/2_pred} &
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/381068411290/0_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/381068411290/1_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/381068411290/2_pred} \\

  %row 1, images
  &\includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/400683688858/0} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/400683688858/1} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/400683688858/2} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car1/0} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car1/1} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car1/2} &
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car2/0} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car2/1} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car2/2} \\
  %row 1, reconstructions
  &\includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/400683688858/0_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/400683688858/1_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/400683688858/2_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car1/0_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car1/1_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car1/2_pred} &
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car2/0_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car2/1_pred} &  
  \includegraphics[width=\wxebay\linewidth,height=\wxebay\linewidth,keepaspectratio]{figures/res_net_ebay/car2/2_pred}  \\ 
 \hline
\end{tabular}

\begin{tabular}{ccccccccccc}

  %row 1, images
  (b) &\includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_121479940920/0} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_121479940920/1} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_171848674141/0} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_171848674141/1} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_131557015145/0} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_131557015145/1} &
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_141495821327/0} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_141495821327/1} &
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_351232469447/0} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_351232469447/1}  \\
  %row 1, reconstructions
  &\includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_121479940920/0_pred} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_121479940920/1_pred} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_171848674141/0_pred} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_171848674141/1_pred} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_131557015145/0_pred} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_131557015145/1_pred} &
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_141495821327/0_pred} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_141495821327/1_pred}  &
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_351232469447/0_pred} &  
  \includegraphics[width=\wxebayfail\linewidth,height=\wxebayfail\linewidth,keepaspectratio]{figures/res_net_ebay/fail_351232469447/1_pred}\\
 
\end{tabular}
\end{center}
\label{fig:ebay}
\caption{(a) Sample reconstructions on real images from the Online Products dataset~\cite{ebay}. Top rows are input image sequences (from left to right). Bottom rows are the reconstructions at each time step. (b) Some failure cases.}
\vspace{\figurevspace}
\end{figure}


==> figures/res_net_multiview/figure.tex <==
\newcommand\wxsn{0.075}
\begin{figure}
% \vspace{\figurevspace}
\begin{center}
\begin{tabular}{ccccccccccc}

  %1
  & \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/4} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/4} \\
  %2
  &\includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/2/4_pred} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/81/4_pred} \\ 

  %3
  (a) &\includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/4} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/4} \\
  %4
  &\includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/93/4_pred} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/127/4_pred} \\ 


  %5
  &\includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/4} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/4} \\
  %6
  &\includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/200/4_pred} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/264/4_pred} \\ 
\iffalse
  %7
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/4} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/4} \\
  %8
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/405/4_pred} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/383/4_pred} \\ 
\fi
\hline

\end{tabular}

\begin{tabular}{ccccccccccc}

  %planes
  (b) &\includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/4} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/0} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/1} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/2} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/3} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/4} \\
  %pred
  &\includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/71/4_pred} &
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/0_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/1_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/2_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/3_pred} &  
  \includegraphics[width=\wxsn\linewidth,height=\wxsn\linewidth,keepaspectratio]{figures/res_net_multiview/455/4_pred} \\
 
\end{tabular}

\end{center}


\label{fig:multiview_visual}
\caption{(a) Sample reconstruction on the ShapeNet testing set. Top rows are input image sequences (from left to right). Bottom rows are the reconstructions at each time step. (b) Failure cases.}
\vspace{\figurevspace}
\end{figure}


==> intro_deprecated.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Summary of the current research
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MVS
Multiview stereo (MVS) has made significant progress over the past years due
in part to global optimization algorithms and a probabilistic volumetric
framework~\cite{kolev_joint,kolev_global}. However, most formulations assume
Lambertian lighting and minimize photo-consistency with smoothness
constraints~\cite{kolev_joint,kolev_global,kostrikov}. Due to such
assumptions, in the presence of specularity, concavities, thin structures, and
low-textured regions, MVS generates a noisy and sparse 3D reconstruction.
Recently, to handle such problems, stronger priors have been incorporated to
MVS and resulted in a robust reconstruction~\cite{bao,dame}. Class specific
priors require a high level understanding of the scene rather than using local
image features. However, since MVS heavily relies on photometric errors, the
system fails when wide-baseline images are used~\cite{bao}.

% Single View
Single view reconstruction or depth map estimation on the other hand requires
different types of algorithms that enforce stronger priors about the geometry of
the scene~\cite{hedau_layout,delage}, or using CAD models as a
prior~\cite{aubry,choy}. Recently, Convolutional Neural Networks (CNN) have
been used for depth or normal estimation and shown a promising direction in
learning a large number of vocabularies of geometric priors and global scene
layouts without explicitly modeling those priors~\cite{eigen_depth,liu_2015}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Observations about human visual system
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Although both problems can benefit from a system that incorporates a prior,
there has been no system that can handle both problems. Human visual system also
does not use different mechanisms for the single view and multiview reconstruction.
When we are given multiple view observations of an object, combined with our
priors, we update the priors using observations and update our prediction
sequentially.

However, humans do not we can make two observations from human visual system that allows us
to unify seemingly disjoint MVS and single view reconstruction: priors and
selective update.

% prior
First, using prior knowledge for reconstruction is a very common scheme
adopted in biological agents~\cite{mamassian,hartung}. We observe common
geometric patterns and such patterns resolve many ambiguities. For instance,
symmetry, convexity, and classification of the shape allow us to resolve
ambiguities that arise in the 3D reconstruction. However, in artificial settings,
we can break such patterns and the phenomenon is called optical
illusion~\cite{changizi}. Such strong priors about geometric shapes help us to
reconstruct objects in the absence of information.

% disjoint problems, selective update
Second, to biological agents, reconstructing an object from a single image or
multiple images are not disjoint problems; rather, multiview is a direct
extension of a single view.  Given one image, we reconstruct the object based
on our prior knowledge and observation from the image to form a posterior
distribution about the shape. Then, we update the posterior as we observe new
images~\cite{mamassian}. If we observe disparity between the posterior
reconstruction and the observation, we selectively update the part that
mismatches our prediction, but we keep the other parts the same.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proposed method
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Unify single view, multi-view reconstruction into one framework
Inspired by these observations, we propose the \textbf{3D Recurrent
Reconstruction Network (3D-RRN)} that combines prior and observation to form a
posterior and generate a 3D reconstruction of an object. The \textbf{3D-RRN} uses
an arbitrary number of views to reconstruct an object including a single view
image and unifies the disjoint single-view and multi-view reconstruction
problems into one reconstruction problem.

% 3D Convolutional LSTMs
To this end, we propose \textbf{3D Convolutional Long Short-Term Memory (LSTM)}
which is a variation of standard LSTM~\cite{lstm}. Unlike a standard Recurrent
Neural Network, LSTM can selectively update hidden representation or
keep the hidden representation by controlling input gate and forget gate. This
property can be used for multi-view 3D reconstruction since it gives a network ability to selectively update posterior given new information. If the
posterior and the information from the current frame mismatch, it can update
the a part of the hidden representation.  Also, the 3D convolutional
LSTMs are placed in a 3D spatial grid structure to inject spatial information
to LSTMs and also to regularize the number of connections.

% Selective update
% The 3D Convolutional LSTMs work by first computing which gates to open using the input and the current state. Based on this information, the hidden representation is updated and selected
% 
% the detailed information about parts that were visible in previous inputs but
% are self-occluded in the current viewpoint. In another word, if the
% network sees a chair from the front view and then from the back (2 viewpoints),
% it first takes all information coming from the front view since the
% hidden representation is initialized as zero and needs to update the hidden
% representations. Next, when we feed the rear view image, the network should
% keep the information about the front view but only update the hidden
% representations that correspond to the back of the chair.  This way, we do not
% corrupt the information about the front view and selectively update the
% information.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Paper structure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!htp]
  \centering
  \includegraphics[width=0.5\textwidth]{overview/voxel_reconstruction_overview}
  \caption{Overview of the \textbf{3D-Recurrent Reconstruction Network}: the
image at each time frame goes through a CNN encoder. The LSTM units take features as an input and combine with previous states to update the hidden states. Next, the decoder 
projects the hidden states to 3D voxel space and outputs final prediction in
the form of probabilistic voxel occupancy map.}
  \label{fig:overview}
\end{figure}

An overview of our reconstruction network is shown in
Figure~\ref{fig:overview}. In Section~\ref{sec:network}, we introduce the 3D
Recurrent Reconstruction Network (3D-RRN) and present 3D Convolutional LSTMs.
In Section~\ref{sec:implementation}, we go over how we generated training data
and details of the training process. Next, we test our approach on various
datasets including PASCAL 3D and ShapeNet in Section~\ref{sec:experiments}.

% In Section.~\ref{sec:overview}, we go over the 3D convolution and 3D
% pooling and the 3D-CNN architectures. In Section.~\ref{sec:result}, we present
% the classification results on the new large 3D shape dataset: ShapeNetCore
% \cite{shapenet2015} and also on Princeton Shape Benchmark \cite{princeton}.
% In Section.~\ref{sec:analysis}, we analyze the neural network in depth using
% various visualization techniques to understand what neurons have learned.
% 
% % ShapeNet
% Recently, ShapeNet \cite{shapenet2015} proposed the largest dataset for 3D
% shapes. A subset ShapeNetCore consists of 55 classes of 3D shapes such as car,
% airplane, etc. with more than 51k unique 3D models. In this work, we trained
% a CNN for shape classification and show the potential of CNN for shape
% analysis.

% In this paper, we prepared training data using ShapeNet\cite{shapenet2015}
% dataset - a richly-annotated, large-scale dataset of 3D shapes - along with
% data augmentation by applying random transformations to the model on the fly.
% Moreover, we trained a 3D convolutional neural network to let the network learn
% the best features over 3D space to classify 3D models. Then, we made a thorough
% analysis of the network to investigate what the network has learned.
% Additionally, we extended this work by extracting additional semantic
% information of the model such as pose.


==> related_works.tex <==
% \subsection{Object-level Single View Reconstruction}
% % Single View
% Object level single view methods have 
% can be categorized into three methods: shape
% from shading, 3D CAD model based method
% 
% Object level single view reconstruction has long been studied. The earliest
% object level detection used a 3D model to match the object exatly~\cite{lowe}.
% 
% Intrinsic image based~\cite{barron}
% Model based Single view reconstruction~\cite{kar, vincent}

\subsection{Priors for Single View and Multi View Reconstruction}

% Single view, Multi-view Reconstruction setting, failure modes
Single view reconstruction and multi-view reconstruction with sparse
viewpoints remain as challenging problems in Computer Vision.

% The ambiguities arise in reconstruction have been dealt using mid-level or
% object-level shape priors.

\paragraph{Multi View Stereo.}
Multi view stereo (MVS) methods that do not use shape priors may 
produce dense and very accurate reconstructions.
% Chris: Danfei, all MVS that I cited on the above requires camera positions as an input \cite{kolev_joint,kolev_global} and all MVS dataset provide the parameters. Below, you cited SFM method. Should we make a clear distinction between the methods?
% However, many MVS frameworks require very accurate camera parameter estimates which is not possible to extract when wide-baseline images are used.
However, they are geometric feature-based
and often heavily rely on matching keypoints across multiple views~\cite{Fitzgibbon1998sfm,dellaert2000sfm,koch2000sfm,lhuillier2005sfm,wu2011sfm}
, camera positions/calibrations~\cite{kolev_joint,kolev_global}, and/or other cues such as silhouettes~\cite{boisvert2013silhouettes} or shading~\cite{wu2011shading}. 
These approaches would fail if the consecutive views are too sparse
or the object surface reflectance function largely deviates from the lambertian assumption. 
On the other hand, volumetric or voxel representation-based methods such as
~\cite{dyer2001volumetric,vogiatzis2007volumetric,tran2006volumetric,hornung2006volumetric,slabaugh2004voxelcoloring,anwar2006voxelcoloring}
require detailed foreground/background segmentation. 
In addition, Space Carving-based methods ~\cite{seitz1999voxelcoloring,broadhurst2001probabilistic} 
may produce surfaces that tend to bulge out in regions of low surface texture. 
Our approach is agnostic to these limitations and can work with few views 
(or as little as just one) with large baselines.


\paragraph{Multi View Stereo with Priors.}

Multi-View Stereo (MVS) systems assume Lambertian lighting and minimize photo-consistency along with smoothness constraints~\cite{kolev_joint,kolev_global,kostrikov}. Also, MVS requires accurate camera matrices for all images and the object has to be placed on a simple background to make the segmentation easier~\cite{mvs_dataset}.

Due to such strong assumptions, if any of the assumptions fails such as presence of specularity, concavities, thin structures, low-textured regions, wide-baseline images, and noisy background, MVS generates a noisy and sparse 3D reconstruction.

Recently, to handle such problems, object-level priors have been incorporated to
MVS and resulted in a robust reconstruction~\cite{bao,dame}. However, those methods still require accurate camera parameters to detect and place the object-level priors. Thus, the systems fail when the baseline across views is too large (15 degree).

Another major issue is that they often rely on adapting 3D shapes from a collection of template
CAD models to the test image which often leads to “over-smoothed" reconstructions~\cite{kar2015category,dame}.

% Our work can identify the viewpoint
Our approach is agnostic to these limitations and can work with few views
(or as little as just one) with large baselines. The system identifies an object and aligns the object with other observations using high-level understanding of the object.


% Single View
\paragraph{Single View Reconstruction.}
Single view reconstruction or depth map estimation on the other hand requires
different types of algorithms that enforce stronger priors about the geometry of
the scene~\cite{hedau_layout,delage}, or using CAD models as a
prior~\cite{aubry,choy} or shading with segmentation mask~\cite{barron}. Recently, Convolutional Neural Networks (CNN) have
been used for depth or normal estimation and shown a promising direction in
learning a large number of vocabularies of geometric priors and global scene
layouts without explicitly modeling those priors~\cite{eigen_depth,liu_2015}.

% single view reconstruction
Single view reconstruction, on the other hand, is inherently an ill-posed problem.
To recover the lost depth during projection, local geometric
shapes and global consistency priors have been widely used for single view
reconstruction. 

\iffalse
The priors used for both single view and multiview reconstruction can be
classified into three categories: local geometric priors, mid-level shape priors
and high-level or class specific priors.

The most popular forms of local geometric priors are Conditional Random Field
(CRF)~\cite{saxena_depth,ladicky_normal,saxena_make3d,sun}. CRF
unary potentials encode the priors about the local geometry, and binary or
high-order edges enforce smoothness.

For mid-level shape priors, \cite{gupta,badino,sinha} used basic geometric
shapes such planes, cuboids or stixels as geometric shapes that reduce the
complexity of the shape.

More complex high-level priors require understanding about the scene or
objects. For artificial structures and indoor scenes, layouts and Manhattan
assumption along with epipolar geometry have been widely used~\cite{delage,hedau}.
For object-level priors, class specific shape priors~\cite{bao,dame,aubry,choy,prisacariu}
allowed accurate 3D reconstruction of the objects.
\fi


Recently, using Convolutional Neural Network (CNN) for single image depth
estimation has shown a promising direction~\cite{eigen_depth} in single view
reconstruction. Compare to shallow models such as MRF or SFM or explicit shape
modeling, neural network learns high-level understanding~\cite{zeiler} which
suits the task. CNN can capture the priors about the objects appearances and we
can project the priors back to image plane or can be transferred to another
image~\cite{zeiler,gatys}.


\iffalse
% multiview reconstruction w/o priors
Multi View Stereo (MVS) has made significant progress methods that do not use prior knowledge about shapes
produce dense and very accurate reconstructions. They heavily rely on
matching keypoints across multiple views~\cite{lhuillier2005sfm,wu2011sfm}
and other cues such as silhouettes~\cite{boisvert2013silhouettes} or
shading~\cite{wu2011shading}.
These approaches would fail if images fail to meet the common assumptions such
as Lambertian lighting, narrow-baseline 

consecutive views are too sparse
or the object surface reflectance function largely deviates from the lambertian assumption.
On the other hand, volumetric or voxel representation-based methods~\cite{dyer2001volumetric,vogiatzis2007volumetric,tran2006volumetric,hornung2006volumetric}
requires a detailed foreground/background segmentation.
In addition, Space Carving-based methods~\cite{seitz1999voxelcoloring,broadhurst2001probabilistic}
may produce surfaces that tend to bulge out in regions of low surface texture.
Our approach is agnostic to these limitations and can work with few views
(or as little as just one) with large baselines.

% multiview reconstruction w priors
There are many recent works addressing the problem of multiview reconstruction 
using shape priors. Some notable examples are ~\cite{bao,sun,dame}.
~\cite{bao} performs reconstruction at the category level by learning
a mean shape prior along with corresponding feature points on the shape from a
set of image point cloud pairs. Then the system matches a input image-point cloud pair
to the learned feature points and by which deformes the mean shape into the given point cloud~\cite{bao}. 
\cite{sun} uses an object-specific Markov Random Field (MRF) to integrate shape priors
for articulated and deformable object reconstruction.
\cite{dame} tackles the dense SLAM problem by detecting known objects in the scene and
improve pose estimation and reconstruction by embedding the shape priors.
% Stereo method
% \cite{guney2015displets} achieves state-of-the-art result in reconstructing cars in
% urban setting by generating disparity proposals using category-specific shape priors.

These methods use shape priors or model-based inference to circumvent
the issue of having feature mismatches due to secularities. However, they still
suffer from issues such as fail to reconstruct when the number
of feature mismatches due to specular reflections is too large or the baseline
across views is too large (i.e. the number of view is too limited). Another major
issue is that they often rely on adapting 3D shapes from a collection of template
CAD models to the test image which often leads to “over-smoothed" reconstructions.
Our work, on the other hand, stores prior knowledge about object shapes in the learnt
weights of the LSTM structure still works when few images (or as a little a single image) are available.
% need more arguments
\fi


\subsection{Recurrent Neural Network}

% RNN
A Recurrent Neural Network (RNN) is a feed forward network that can process a
variable-length input and output. The critical part of RNN is the hidden layers
(like the Hidden Markov Model hidden state) whose activation at each time step
depends on the previous inputs. At each time step, the hidden layer process the
input and update the hidden state. However, naive recurrence fails to capture
long-term dependency~\cite{lstm}. To mitigate the problem, Hochreiter et
al.~\cite{lstm} proposed Long Short-Term Memory (LSTM) which includes controlling
units for input and output. The controlling units, or gating units, allow the
network to selectively update or keep the hidden state. Recently, several
variations of LSTM has been proposed. Most notably, Gated Recurrent Unit
(GRU), first proposed for machine translation, works better than LSTM in this
type of problems~\cite{gru}.

